The GTC exoplanet transit spectroscopy survey II: An overly-large Rayleigh-like feature for exoplanet TrES-3b

We set to search for Rayleigh scattering and K and Na absorption signatures from the atmosphere of TrES-3b using ground-based transmission spectroscopy covering the wavelength range from 530 to 950 nm as observed with OSIRIS@GTC. Our analysis is based on a Bayesian approach where the light curves covering a set of given passbands are fitted jointly with PHOENIX-calculated stellar limb darkening profiles. The analysis is carried out assuming both white and red -- temporally correlated -- noise, with two approaches (Gaussian processes and divide-by-white) to account for the red noise. An initial analysis reveals a transmission spectrum that shows a strong Rayleigh-like increase in extinction towards the blue end of the spectrum, and enhanced extinction around the K I resonance doublet near 767 nm. However, the signal amplitudes are significantly larger than expected from theoretical considerations. A detailed analysis reveals that the K I-like feature is entirely due to variability in the telluric O$_2$ absorption, but the Rayleigh-like feature remains unexplained.

==> commands.tex <==
\newcommand{\emth}[1]{\ensuremath{#1}\xspace}
\newcommand{\parm}[1]{\ensuremath{\theta_\mathrm{#1}}\xspace}

\newcommand{\covmat}{\emth{\boldsymbol{\Sigma}}}

\newcommand{\npb}{\emth{n_\mathrm{pb}}}
\newcommand{\nph}{\emth{n_\mathrm{ph}}}
\newcommand{\nip}{\emth{n_\mathrm{\mu}}}

\newcommand{\gcm}{\emth{\mathrm{g\,cm^{-3}}}}
\newcommand{\mjup}{\emth{\mathrm{M_{Jup}}}} 	% Jupiter mass
\newcommand{\rjup}{\emth{\mathrm{R_{Jup}}}} 	% Jupiter radius
\newcommand{\mearth}{\emth{\mathrm{M_{\oplus}}}} 	% Jupiter mass

\newcommand{\logg}{log {\it g}}
\newcommand{\met}{[M/H]}

\newcommand{\ud}{\ensuremath{\mathrm{d}}}
\newcommand{\lh}{\ensuremath{\ell}}
\newcommand{\llh}{\ensuremath{\ln P}}
\newcommand{\iid}{i.i.d.\xspace}

\newcommand{\pvec}{\ensuremath{\boldsymbol{\theta}}\xspace}
\newcommand{\Dlc}{\ensuremath{\vec{D_{\mathrm{LC}}}}\xspace}
\newcommand{\Drv}{\ensuremath{\vec{D_{\mathrm{RV}}}}\xspace}
\newcommand{\Dld}{\ensuremath{\vec{D_{\mathrm{LD}}}}\xspace}

\newcommand{\UP}[1]{\ensuremath{U(#1)}\xspace}
\newcommand{\NP}[1]{\ensuremath{N(#1)}\xspace}

\newcommand{\pfr}{\parm{f}}           		% Flux ratio
\newcommand{\prr}{\parm{k}}           		% Radius ratio
\newcommand{\pper}{\parm{p}}          		% Period
\newcommand{\pa}{\parm{a}}            		% Semi-major axis
\newcommand{\pec}{\parm{e}}           		% Eccentricity
\newcommand{\pom}{\parm{\omega}}      		% Argument of periastron
\newcommand{\pin}{\parm{i}}           		% Inclination
\newcommand{\ptc}{\parm{tc}}
\newcommand{\ldu}{\parm{u}}
\newcommand{\ldv}{\parm{v}}
\newcommand{\prho}{\parm{\rho}} 

\newcommand{\pbl}{\parm{B}}			% Baseline
\newcommand{\pext}{\parm{x}}			% Extinction coefficient
\newcommand{\pcf}{\parm{c}}       		% Contamination
\newcommand{\pip}{\parm{b}}	                % Impact parameter

\newcommand{\smass}{\emth{\mathrm{M_\star}}}
\newcommand{\srad}{\emth{\mathrm{R_\star}}}
\newcommand{\pmass}{\emth{\mathrm{M_P}}}	% Planet mass
\newcommand{\prad}{\emth{\mathrm{R_P}}}	% Planet radius

\newcommand{\Tbr}{\emth{T_{\mathrm{br}}}}  	% Brightness temperature
\newcommand{\Teq}{\emth{T_{\mathrm{eq}}}}	% Equilibrium temperature

\newcommand{\Age}{\emth{A_{\mathrm{g}}}} 	% Geometric albedo
\newcommand{\Abo}{\emth{A_{\mathrm{B}}}} 	% Bond albedo

\newcommand{\bayesf}{\emth{B_{\mathrm{10}}}} 	% Bayes factor

\newcommand{\kobs}{\emth{k_\mathrm{obs}}}
\newcommand{\teff}{\emth{T_\star}}
\newcommand{\kreal}{\emth{k_\mathrm{real}}}
\newcommand{\tcont}{\emth{T_\mathrm{c}}}
\newcommand{\tspot}{\emth{T_\mathrm{s}}}
\newcommand{\tstar}{\emth{T_\star}}
\newcommand{\rstar}{\emth{R_\star}}

\newcommand{\placeholder}[2]{\vspace*{#1}\begin{center} -- PLACEHOLDER --\\#2\end{center}\vspace*{#1}}
